A Hybrid control approach to the route planning problem for sailing boats

We present an optimal hybrid control approach to the problem of stochastic route planning for sailing boats, especially in short course fleet races, in which minimum average time is an effective performance index. We show that the hybrid setting is a natural way of taking into account tacking/gybing maneuvers and other discrete control actions, and provide examples of increasing complexity to model the problem. Moreover, we carry out a numerical validation of the approach and show that results are in good agreement with theoretical and practical knowledge.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
%\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
\newcommand{\TheTitle}{A hybrid control approach to the route planning problem for sailing boats} 
\newcommand{\TheAuthors}{R. Ferretti and A. Festa}

% Sets running headers as well as PDF title and authors
\headers{Route planning problem for sailing boats}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors \today.}}

% Authors: full names plus addresses.
\author{Roberto Ferretti \thanks{Dipartimento di Matematica e Fisica, Universit\`a Roma Tre, L.go S. Leonardo Murialdo, 1, 00146 Roma, Italy. \email{ferretti@mat.uniroma3.it}} \and Adriano Festa \thanks{INSA Rouen,
LMI laboratory, Avenue de l'Universit\'e, 76800 Saint-\'Etienne-du-Rouvray, France. \email{adriano.festa@insa-rouen.fr}}
}






\newcommand{\ep}{\varepsilon}
\newcommand{\eps}[1]{{#1}_{\varepsilon}}
%%%%%%%%%%%%%% My Macros %%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator{\diver}{div}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\atan2}{atan2}
\DeclareMathOperator{\R}{\mathbb{R}}
\DeclareMathOperator{\PP}{\mathbb{P}}
\DeclareMathOperator{\Q}{\mathbb{Q}}
\DeclareMathOperator{\A}{\mathcal{A}}
\DeclareMathOperator{\T}{\mathcal{T}}
\DeclareMathOperator{\Z}{\mathbb{Z}}
\DeclareMathOperator{\N}{\mathbb{N}}
\DeclareMathOperator{\de}{\!\nabla\!}
\DeclareMathOperator{\io}{\int_\Omega}
\DeclareMathOperator{\perogni}{\;\;\;\:\, \forall}
\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\sen}{sen}
\DeclareMathOperator{\loc}{loc}
\DeclareMathOperator{\co}{co}
\providecommand{\norm}[1]{\lVert#1\rVert}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\G}{\Gamma}
\newcommand{\dt}{\Delta t}
\newcommand{\hk}{{hk}}
\newcommand{\HH}{{\mathbb H}}
\newcommand{\V}{{\mathbb V}}
\newcommand{\E}{{\mathbb E}}
\newcommand{\I}{{\mathcal I}}
\newcommand{\RN}{{\mathbb R^N}}
\newcommand{\RR}{{\mathbb R}}
%\newcommand{\C}{{\mathbb C}}
\DeclareMathOperator*{\medcup}{\mathbin{\scalebox{0.85}{\ensuremath{\bigcup}}}}
\newcommand{\zz}{{\mathbb z}}

\newcommand{\bO}{{\mathbb O}}
\newcommand{\bM}{{\mathbb M}}
\newcommand{\bL}{{\mathbb L}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cA}{{\mathcal A}}
\newcommand{\ccB}{{\mathcal B}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\wtM}{{\widetilde M}}
\newcommand{\wtU}{{\widetilde U}}
\newcommand{\wtlambda}{{\widetilde \lambda}}
\newcommand{\whM}{{\widehat M}}


% grec
\renewcommand{\phi}{\varphi}
\renewcommand{\a}{{\alpha}}
\renewcommand{\b}{{\beta}}
\newcommand{\g}{{\gamma}}
\renewcommand{\d}{{\delta}}
\newcommand{\e}{\epsilon}
\renewcommand{\k}{\kappa}
\renewcommand{\l}{\lambda}
\newcommand{\om}{\omega}
\newcommand{\s}{{\sigma}}
\renewcommand{\th}{\theta}
\newcommand{\Th}{\Theta}

\newcommand{\Exp}{{^}}
\newcommand{\deter}{\hbox{det}}
\newcommand{\Ker}{\ker}
\newcommand{\conv}{\hbox{conv}}
\newcommand{\pd}{\partial}
\newcommand{\Dx}{{\Delta x}}





\newcommand{\tv}{{\tilde v}}

\newcommand{\Lh}{\mathcal{L}_h}
\newcommand{\ds}{\displaystyle}
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}
%\def\qed{\ifmmode\else\unskip\quad\fi\squareforqed}
%\def\smartqed{\def\qed{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
%\penalty50\hskip1em\null\nobreak\hfil\squareforqed
%\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}}
\newcommand{\supp}{\mathrm{supp}\;}
\newcommand{\db}{\mathbf{d}}





%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

